Financial Time Series Forecasting with Deep Learning : A Systematic Literature Review: 2005-2019

Financial time series forecasting is, without a doubt, the top choice of computational intelligence for finance researchers from both academia and financial industry due to its broad implementation areas and substantial impact. Machine Learning (ML) researchers came up with various models and a vast number of studies have been published accordingly. As such, a significant amount of surveys exist covering ML for financial time series forecasting studies. Lately, Deep Learning (DL) models started appearing within the field, with results that significantly outperform traditional ML counterparts. Even though there is a growing interest in developing models for financial time series forecasting research, there is a lack of review papers that were solely focused on DL for finance. Hence, our motivation in this paper is to provide a comprehensive literature review on DL studies for financial time series forecasting implementations. We not only categorized the studies according to their intended forecasting implementation areas, such as index, forex, commodity forecasting, but also grouped them based on their DL model choices, such as Convolutional Neural Networks (CNNs), Deep Belief Networks (DBNs), Long-Short Term Memory (LSTM). We also tried to envision the future for the field by highlighting the possible setbacks and opportunities, so the interested researchers can benefit.

==> tables/nomenclature.tex <==
\begingroup
\footnotesize

\fontsize{7}{9}\selectfont
\begin{longtable}{
                p{0.06\linewidth}
                p{0.22\linewidth}
                p{0.06\linewidth}
                p{0.22\linewidth}
                p{0.08\linewidth}
                p{0.22\linewidth}
                }


%\caption{Nomenclature}\\
%\label{table:nomenclature}\\

\hline
\textbf{Abbr.}                                                          & 
\textbf{Explanation}                                                       &
\textbf{Abbr.}                                                       & 
\textbf{Explanation}                                                  &
\textbf{Abbr.}                                                       & 
\textbf{Explanation}                                                  \\ 
\hline
\endhead 
 \hline

% INSERT TABLE DATA HERE
AAR & Annual Rate of Return & FTSE & London Financial Times Stock Exchange Index & PCC & Pearson’s Correlation Coefficient \\ \hline
AC & Autocorrelation & GA & Genetic Algorithm & PCD & Percentage of Correct Direction \\ \hline
AE & Autoencoder & GAF & Gramian Angular Field & PLR & Piecewise Linear Representation \\ \hline
AMEX & American Stock Exchange & GAN & Generative Adversarial Networks & PNN & Probabilistic NN \\ \hline
ANN & Artificial Neural Network & GAN-D & Direction Prediction Loss & POCID & Percentage of Change in Direction \\ \hline
AR & Active Return & GAN-F & Forecast Error Loss & PPO & Proximal Policy Optimization  \\ \hline
ARCH & Auto-Regressive Conditional Heteroscedasticity & GARCH & Generalised Auto-Regressive Conditional Heteroscedasticity & PROFIT & Average Annual Profit of the Model \\ \hline
ARIMA & Autoregressive Integrated Moving Average  & GBDT & Gradient-Boosted-DecisionTrees  & PSN & Psi-Sigma Network \\ \hline
ATR & Average True Range & GLM & Generalized Linear Model & PSO & Particle Swarm Optimization \\ \hline
AUC & Area Under the Curve & G-mean & Geometric Mean & r1 & Correlation coefficient between actual value and prediction value \\ \hline
AUROC & Area Under the Receiver Operating Characteristics & GP  & Genetic Programming & r2 & Correlation coefficient between actual return and prediction return \\ \hline
BA & Balanced Accuracy & GPU & Graphic Processing Unit & $R^2$ & Squared correlation, Non-linear regression multiple correlation
coefficient \\ \hline
BELM & Basic Extreme Learning Machine & GRU & Gated-Recurrent Unit & RA & Rolling Average \\ \hline
BETC & Break Even Transaction Cost & GSPC & S\&P500 Commodity Price Index & RAF, RF & Random Forests  \\ \hline
BIST & Istanbul Stock Exchange Index & HAN & Hybrid Attention  Network & RBF & Radial Basis Function Neural Network \\ \hline
Bi-GRU & Bidirectional Gated Recurrent Unit & HFT & High Frequency Trading & RBM & Restricted Boltzmann Machine \\ \hline
BOLL & Bollinger Band & HIT, HR & Hit Rate & RCEFLANN & Recurrent Computationally Efficient Functional Link Neural Network \\ \hline
BP & Back Propagation & HMRPSO & Modified Version of PSO  & RCI & Rank Correlation Index \\ \hline
BPTT & Back Propagation Through Time & HS300 Index & China Shanghai Shenzhen 300 Stock Index & RELU & REctified Linear Unit \\ \hline
BSE & Bombay Stock Exchange & HSI & Hong Kong stock market index (Hang Seng Index) & RETURN & Average Annual Returns of the Model \\ \hline
CAGR & Compound Annual Growth Rate & IBB & iShares Nasdaq Biotechnology ETF & RMSE & Root Mean Square Error \\ \hline
CAR & Cumulative Abnormal Return & IC & Information Coeffiencient & RMSRE & Root Mean Square Relative Error \\ \hline
CART & Classification and Regression Trees & IR & Information Ratio & RNN & Recurrent Neural Network \\ \hline
CC & Correlation Coefficient & ISE100 & Istanbul Stock Exchange Index & ROA  & Return on Assets \\ \hline
CCI & Commodity Channel Index & IXIC & NASDAQ Composite Index & ROC & Price of Change \\ \hline
CDAX & German Stock Market Index Calculated by Deutsche Börse & KELM & Kernel Extreme Learning Machine & RSE & Relative Squared Error \\ \hline
CDBN-FG & Fuzzy Granulation with Continuous-valued Deep Belief Networks & KOSPI & The Korea Composite Stock Price Index & RSI & Relative Strength Index \\ \hline
CDS & Credit Default Swaps & KS & Kolmogorov–Smirnov & S\&P500 & Standard’s \& Poor’s 500 Index \\ \hline
CGAN & Conditional GAN & LAR & Linear Auto-regression Predictor & SAE & Stacked Autoencoder \\ \hline
CEW & Emerging Markets Currency Index & LDA & Latent Dirichlet Allocation & SAR & Parabolic Stop and Reverse \\ \hline
CME & Chicago Mercantile Exchange & LFM & Lookahead Factor Models & SCI & SSE Composite Index  \\ \hline
CNN & Convolutional Neural Network & LOB & Limit Order Book Data & SD & Standard Deviation (also referred as the Greek letter r) \\ \hline
CRSP & Center for Research in Security Prices  & LRNFIS & Locally Recurrent Neuro-fuzzy Information System & SDAE & Stacked Denoising Autoencoders \\ \hline
CSE & Colombo Stock Exchange  & LSTM & Long Short Term Memory & SFM & State Frequency Memory \\ \hline
CSI & China Securities Index  & MA & Moving Average & SGD & Stochastşc Gradient Descent \\ \hline
cWN & Conditional Wavenet  & MACD & Moving Average Convergence and Divergence & SI & Stochastic Index \\ \hline
DA & Direction Accuracy & MAD & Mean Absolute Deviation & SLP & Single Layer Perceptron \\ \hline
DAX & The Deutscher Aktienindex  & MADR & Moving Average Deviation Rate & SMAPE & Symmetric Mean Absolute Percentage Error \\ \hline
DBN & Deep Belief Network & MAE & Mean Absolute Error & SOM & Self-Organising Map \\ \hline
DDPG & Deep Deterministic Policy Gradient & MAM & Moving Average Mapping & SR & Sharpe-ratio \\ \hline
DE & Differential Evolution & MAP & Maximum Absolute Percentage Error & SSE & Shanghai Stock Exchange \\ \hline
DeepCNL & Deep Co-investment Network Learning & MAPE & Mean Absolute Percentage Error & SVM & Support Vector Machine \\ \hline
DCNN & Deep Convolutional Neural Network & MAR & Mean Abnormal Return & SVR & Support Vector Regression \\ \hline
Deep-FASP & The Financial Aspect and Sentiment Prediction task with Deep neural networks & MASE & Mean Standard Deviation & SVD & Singular Value Decomposition \\ \hline
DFFN & Deep Feed Forward Network & MC  & Monte Carlo & SZSE & Shenzhen Stock Exchange Composite Index  \\ \hline
DGM & Deep Neural Generative Model & MCC & Matthew Correlation Coefficient  & TAIEX & Taiwan Stock Exchange Capitalization Weighted Stock Index \\ \hline
DJIA & Dow Jones Industrial Average & MDA & Multilinear Discriminant Analysis  & TALIB & Technical Analysis Library Package \\ \hline
DL  & Deep Learning  & MDD & Maximum Drawdown & TAR-VEC & Threshold Autoregressive Vector Error Correction model \\ \hline
DLR & Deep Learning Representation & MDP & Markov Decision Process & TD  & Temporal Difference \\ \hline
DMLP & Deep Multi Layer Perceptron & MFI & Money Flow Index & TDNN & Timedelay NN \\ \hline
DMI & Directional Movement Index & MI & Mutual Information & THEIL-U, TIC & Theil's inequality coefficient \\ \hline
DNN & Deep Neural Network & ML  & Machine Learning & TN & True Negative \\ \hline
DOF & Degrees of Freedom & MLP & Multilayer Perceptron & TP & True Positive \\ \hline
DP & Dynamic Programming & MODRL & Multi-objective Deep Reinforcement Learning & TR & Total Return \\ \hline
DPA & Direction Prediction Accuracy & MoE & Mixture of Experts & true & True Range of Price Movements \\ \hline
DRL & Deep Reinforcement Learning & MOEA & Multiobjective Evolutionary Algorithms & TUNINDEX & Tunisian Stock Market Index \\ \hline
DRSE & Deep Random Subspace Ensembles & MSE & Mean Squared Error & TSE & Tokyo Stock Exchange  \\ \hline
DTW & Dynamic Time Warping & MSFE & Mean Squared Forecast Error & TWSE & Taiwan Stock Exchange  \\ \hline
DQL & Deep Q-Learning & MSPE & Mean Squared Prediction Error & uWN & Unconditional WaveNet \\ \hline
EA & Evolutionary Algorithms & MTM & Momentum & VAR & Vector Auto Regression \\ \hline
EC & Evolutionary Computation & NARMAX & Nonlinear Autoregressive Moving Average model with exogenous inputs & VIX & S\&P500 Volatility Index \\ \hline
EMD2FNN & Empirical Mode Decomposition and Factorization Machine based Neural Network & NASDAQ & National Association of Securities Dealers Automated Quotations & VR & Variance Reduction \\ \hline
EMA & Exponential Moving Average & NES & Natural Evolution Strategies  & VXD & Dow Jones Industrial Average Volatility Index  \\ \hline
ETF & Exchange-traded Fund & NIFTY & National Stock Exchange of India & VXN & NASDAQ100 Volatility Index \\ \hline
FAR & False Acceptance Rate & NIKKEI & Tokyo Nikkei Index & VWL & WL Kernel-based Method \\ \hline
FDDR & Fuzzy Deep Direct Reinforcement Learning & NLP & Natural Language Processing & WBA & Weighted Balanced Accuracy \\ \hline
FE-QAR & Fixed Effects Quantile VAR & NMAE & Normalized Mean Absolute Error & WEKA & Waikato Environment for Knowledge Analysis \\ \hline
FiQA & Financial Opinion Mining and Question Answering Challange & NMSE & Normalized Mean Square Error & WHR & Weighted Hit Rate \\ \hline
FN & False Negative & NYMEX & New York Mercantile Exchange & WMTR & Weighted Multichannel Time-series Regression \\ \hline
FNN & Fully Connected Neural Network & NYSE & New York Stock Exchange & WPR & William \% R \\ \hline
FP & False Positive & OBV & On Balance Volume & WSURT & Wilcoxon Sum-rank Test  \\ \hline
FPE & Akaike’s Minimum Final Prediction Error & OCHL & Open,Close,High, Low & WT & Wavelet Transforms \\ \hline
FPGA & Field Programmable Gate Array & OCHLV & Open,Close,High, Low, Volume  &  &  \\ \hline
FRR & False Rejection Rate & PCA & Principal Component Analysis &  &  \\ \hline





\end{longtable}
\endgroup

==> tables/top_journals.tex <==
\begingroup
\footnotesize
\fontsize{7}{9}\selectfont
\begin{longtable}{lcc}
            
              

\caption{Top Journals}\\
\label{table:top_journals}\\


\hline
   &
\textbf{All-years count}   &
\textbf{Last-3-years count}    \\ 
\hline
\endhead 



Expert Systems with Applications & 7 & 5 \\ \hline
Neurocomputing & 3 & 1 \\ \hline
Applied Soft Computing & 2 & \\ \hline
The Journal of Supercomputing & 2 & 2 \\ \hline
Decision Support Systems & 2 & 1 \\ \hline
Knowledge-based Systems & 2 & 2 \\ \hline
European Journal of Operational Research & 2 & 2 \\ \hline
IEEE Access & 2 & 2 \\ \hline
IEEE Transactions on Neural Networks & 2 & \\ \hline
Algorithmic Finance & 1 & \\ \hline
Journal of King Saud University – Computer and Information Sciences & 1 & 1 \\ \hline
Journal of Mathematical Finance & 1 & 1 \\ \hline
Mathematical Problems in Engineering & 1 & 1 \\ \hline
Multimedia Tools and Applications & 1 & \\ \hline
Neural Computing and Applications & 1 & 1 \\ \hline
Neural Computing and Applications & 1 & 1 \\ \hline
Resources Policy & 1 & \\ \hline
Pattern Recognition Letters & 1 & \\ \hline
Plos One & 1 & 1 \\ \hline
Journal of Econometrics & 1 & \\ \hline
Review of Financial Economics & 1 & \\ \hline
Romanian Economic Business Review & 1 & \\ \hline
SSRN - Social Science Research Network & 1 & 1 \\ \hline
Systems Engineering - Theory \& Practice & 1 & \\ \hline
The Journal of Finance and Data Science & 1 & \\ \hline
Journal of International Financial Markets, Institutions \& Money & 1 & \\ \hline
International Journal of Machine Learning and Computing & 1 & 1 \\ \hline
Journal of Computational Finance & 1 & 1 \\ \hline
IEEE Transactions on Knowledge and Data Engineering & 1 & 1 \\ \hline
Concurrency and Computation Practice and Experience & 1 & 1 \\ \hline
Data \& Knowledge Engineering & 1 & 1 \\ \hline
Electronic Commerce Research and Applications & 1 & 1 \\ \hline
Energy Economics & 1 & 1 \\ \hline
Engineering Letters & 1 & 1 \\ \hline
Frontiers in Signal Processing & 1 & 1 \\ \hline
IEEE Transactions on Industrial Informatics & 1 & 1 \\ \hline
IEEE Transactions on Neural Networks and Learning Systems & 1 & 1 \\ \hline
Journal of Business Economics and Management & 1 & \\ \hline
IEICE Transactions on Information and Systems & 1 & 1 \\ \hline
International Journal of Mathematics and Computers in Simulation & 1 & 1 \\ \hline
Innovative Infotechnologies for Science, Business and Education & 1 & \\ \hline
International Journal of Economics and Management Systems & 1 & \\ \hline
International Journal of Forecasting & 1 & \\ \hline
International Journal of Intelligent Systems and Applications in Engineering & 1 & 1 \\ \hline
Algorithms & 1 & 1 \\ \hline
Wireless Personal Communications & 1 & 1 \\ \hline





\end{longtable}
\endgroup
